Attention Sink in Transformers: A Survey on Utilization, Interpretation, and Mitigation

As the foundational architecture of modern machine learning, Transformers have driven remarkable progress across diverse AI domains. Despite their transformative impact, a persistent challenge across various Transformers is Attention Sink (AS), in which a disproportionate amount of attention is focused on a small subset of specific yet uninformative tokens. AS complicates interpretability, significantly affecting the training and inference dynamics, and exacerbates issues such as hallucinations. In recent years, substantial research has been dedicated to understanding and harnessing AS. However, a comprehensive survey that systematically consolidates AS-related research and offers guidance for future advancements remains lacking. To address this gap, we present the first survey on AS, structured around three key dimensions that define the current research landscape: Fundamental Utilization, Mechanistic Interpretation, and Strategic Mitigation. Our work makes a pivotal contribution by highlighting the key concepts and main trends in the field, guiding researchers through the evolution of AS-related studies. We envision this survey as a valuable resource, empowering researchers to effectively manage AS within the current Transformer paradigm, while simultaneously inspiring innovative advancements for the next generation of Transformers. The paper list of this work is available at https://github.com/ZunhaiSu/Awesome-Attention-Sink.

==> Attention_Sink_in_Transformers/3_Utilization/5_Others.tex <==

Example:



\begin{tcolorbox}[takeawaysbox]
{\large \textbf{\textcolor{TikTokPink}{\textit{Key Takeaways:}}}}
  \begin{enumerate}[leftmargin=*, label=\arabic*)]
    \item \textbf{Core Methodology:} Attention Sinks are established as a foundational, exploitable component in Transformers. Their core property — attracting disproportionate attention — enables systematic model manipulation, forming a unified theoretical lens for diverse research.

    \item \textbf{Practical Approaches:} This manipulation manifests in three distinct ways: as a \textit{vulnerable gateway} for security attacks, a \textit{stabilizing anchor} for enhancing robustness and reducing hallucination, and a \textit{computational knob} for improving efficiency through pruning or bias removal.

    \item \textbf{Synthesis and Perspectives:} The paradigm reveals a central trade-off: sinks provide stability at the cost of potential redundancy and bias. Future work lies in developing \textit{adaptive sink management} to dynamically optimize this balance, transforming sinks from ad-hoc targets into core, controllable model parameters.
  \end{enumerate}
\end{tcolorbox}

% --- Methodological Formulation ---
\subsubsection{Methodological Formulation}
This survey synthesizes ten recent studies under a unifying conceptual framework: the strategic exploitation of the \textbf{Attention Sink}. We define the Attention Sink as a specialized token (e.g., initial tokens, [CLS], or learnable registers) that consistently attracts disproportionately high attention irrespective of semantic content. We posit that it serves as a fundamental yet malleable computational primitive within Transformer-based models. Its intrinsic properties—acting as a stable, high-norm attractor within the attention dynamics—enable three distinct and logically coherent modes of manipulation for downstream objectives:

\begin{enumerate}[label=\textbf{Mode \arabic*}:, leftmargin=*, align=left]
    \item \textbf{The Offensive Gateway.} The sink is weaponized as a \textit{vulnerable entry point} or a \textit{latent trigger}. Its stable, high-attention profile renders it an ideal substrate for injecting malicious functionalities (e.g., backdoors during unlearning) or for eliciting specific, unintended model behaviors (e.g., hallucinations) with minimal, targeted perturbation.
    \item \textbf{The Defensive Anchor.} The sink is \textit{fortified or repurposed} as a stabilizing computational buffer. This is achieved either by enhancing its intrinsic capacity to aggregate salient information (e.g., visual features) or by introducing secret, robust tokens designed to function as protective sinks. This mode directly improves model resilience against errors (e.g., hallucinations) and adversarial perturbations.
    \item \textbf{The Efficiency Knob.} The sink is \textit{systematically identified, optimized, or removed} to eliminate computational redundancy. This encompasses strategies such as actively selecting informative tokens over sink-like redundant ones, evicting less critical tokens from key-value caches, or explicitly excising the sink bias to unlock latent model capabilities without additional training.
\end{enumerate}

% --- Practical Approaches ---
\subsubsection{Practical Approaches}
The following section delineates how each cited work concretely instantiates one of the three methodological paradigms, demonstrating the practical leverage of Attention Sink properties.

\textbf{1. The Offensive Gateway}
\begin{itemize}
    \item \textbf{Backdooring Unlearning \cite{shang2025forgetting}:} This work exposes Attention Sinks as critical gateways for implanting backdoors during the LLM unlearning process. By strategically positioning trigger tokens at these sink positions (e.g., sequence beginnings), a backdoor is embedded that remains dormant under normal conditions but triggers the recovery of “forgotten” knowledge. The attack's success is quantitatively linked to the elevated attention value $A_{\text{sink}}$ garnered by the trigger.
    \item \textbf{Eliciting Hallucination Attacks \cite{wang2025mirage}:} This study demonstrates that targeted manipulation of Attention Sinks (notably initial tokens) in MLLMs can be weaponized to actively induce hallucinations. The attack crafts adversarial inputs that artificially amplify the sink's dominance, thereby hijacking the attention distribution $P_{\text{attn}}$ and diverting it from the veridical visual evidence.
\end{itemize}

\textbf{2. The Defensive Anchor}
\begin{itemize}
    \item \textbf{Alleviating Hallucinations in LVLMs \cite{zhang2025shallow, zhang2024seeing}:} These studies identify a strong correlation between dense visual attention sinks in \textit{shallow model layers} and reduced hallucination propensity. They propose training-free interventions (EVAS/EAH) that amplify this beneficial sink phenomenon by broadcasting the attention map $\mathbf{A}_{\text{sink-head}}$ from the densest sink head to other heads in the same layer, thereby reinforcing the model's visual grounding.
    \item \textbf{Enhancing Adversarial Robustness \cite{pulfer2024robustness}:} This approach introduces secret, learnable \textit{Robustness Tokens} prepended to the input sequence. Optimized via a dual-objective loss $\mathcal{L} = \mathcal{L}_{\text{inv}} + \mathcal{L}_{\text{adv}}$, these tokens evolve into robust “sinks” that stabilize the feature manifold against adversarial perturbations, ensuring clean and adversarial inputs are mapped to proximate representations.
    \item \textbf{Improving OOD Generalization \cite{yellapragada2025leveraging}:} This work harnesses \textit{register tokens}—a form of engineered sinks in Vision Transformers (ViTs)—to isolate high-norm, potentially disruptive patch tokens. The aggregated register embedding $\mathbf{r} = \frac{1}{N}\sum_i \mathbf{r}_i$ is fused with the standard [CLS] token to construct a more robust and generalizable feature representation for downstream classification, enhancing out-of-distribution (OOD) performance.
\end{itemize}

\textbf{3. The Efficiency Knob}
\begin{itemize}
    \item \textbf{Fine-Grained Sparse Attention \cite{chen2025omnisparse}:} OmniSparse implements a dynamic token classification mechanism, labeling queries as either “lazy” (functionally redundant, sink-like) or “active,” followed by pruning the former. Coupled with KV cache slimming, it systematically identifies and removes tokens that contribute minimally beyond base-level attention, achieving acceleration through budget-aware computation.
    \item \textbf{KV Cache Eviction \cite{park2025keydiff}:} KeyDiff formulates cache eviction as an optimization problem based on key vector similarity. Tokens exhibiting high key similarity to others (indicative of low distinctiveness and potential sink-like redundancy) are prioritized for eviction under fixed memory budgets, formally aiming to retain the subset that maximizes overall key diversity.
    \item \textbf{Long Context Compression \cite{li2024streamingdialogue}:} This method learns to compress extended dialogue histories by identifying and preserving critical “information sink” tokens—those that act as semantic hubs for the context—while aggressively compressing peripheral tokens, thus minimizing information loss.
    \item \textbf{Eliminating Sink Bias for Encoding \cite{lin2025look}:} This work diagnoses the initial token's role as a dominant, performance-harming attention sink in autoregressive LLMs used for encoding. By adopting a bidirectional attention paradigm and removing the initial token (the \textit{“No Sink”} strategy), it neutralizes this architectural bias, unlocking the model's intrinsic capability as a high-quality text encoder without any parameter updates, formally expressed as $\text{Encoder}(X) = \text{LLM}(X \setminus \{\text{sink-token}\})$.
\end{itemize}

% --- Synthesis and Perspectives ---
\subsubsection{Synthesis and Perspectives}

\textbf{Advantages of the Sink-Centric View}
\begin{itemize}
    \item \textbf{Unifying Explanatory Power:} It furnishes a parsimonious yet powerful principle that coherently explains a wide spectrum of phenomena and engineering techniques spanning model efficiency, security, and capability enhancement.
    \item \textbf{Pragmatic Intervention Point:} The sink constitutes a highly actionable intervention point within the model's computational graph. Subtle, targeted manipulations (e.g., reinforcement, attenuation, or poisoning) can induce significant and predictable behavioral shifts, offering high leverage for both attack and defense.
    \item \textbf{Bridging Theory and Practice:} This framework effectively connects the foundational theoretical observation of the “attention sink” phenomenon to a diverse suite of cutting-edge, practical algorithms and solutions, demonstrating its translational value.
\end{itemize}

\textbf{Limitations and Open Challenges}
\begin{itemize}
    \item \textbf{Dynamic and Contextual Sinks:} Prevailing approaches often treat sinks as static entities. However, their identity, strength, and role are likely context-dependent. Methodologies for the dynamic identification and adaptation to these “sink dynamics” remain an open area.
    \item \textbf{Theoretical Underpinnings:} The field lacks a rigorous theoretical framework to quantify concepts like “sink capacity” or to formally characterize the Pareto-optimal trade-offs between sink manipulation (for security/robustness) and core model utility/efficiency.
    \item \textbf{Generalization Across Architectures:} Current research is predominantly centered on classical Transformer variants (encoder-decoder/decoder-only). The manifestation and utility of sink-like phenomena in emerging architectures (e.g., State Space Models like Mamba, or hybrid models) are largely uncharted territory.
\end{itemize}

\textbf{Future Directions}
\begin{itemize}
    \item \textbf{Towards Holistic and Adaptive Sink Management:} Future systems may necessitate intelligent controllers that dynamically decide, on a per-input and per-layer basis, whether to \textit{fortify, prune, or ignore} sink tokens, optimizing for a multi-objective function balancing efficiency, robustness, and task accuracy.
    \item \textbf{Sink as a Core Evaluation Metric:} Quantifiable properties of attention sinks (e.g., spatial density, temporal stability, norm distribution) could be standardized as novel diagnostic metrics for benchmarking model robustness (against hallucinations, adversarial attacks) and inference-time efficiency.
    \item \textbf{Formalizing and Optimizing Inherent Trade-offs:} A critical research frontier involves formally modeling the intrinsic tension between maintaining sinks for numerical stability and representation coherence versus removing them to enhance efficiency and mitigate representational bias, followed by developing optimization strategies for this trade-off.
\end{itemize}

==> Attention_Sink_in_Transformers/4_Interpretation/5_Structural_Bias.tex <==


\begin{tcolorbox}[takeawaysbox]
{\large \textbf{\textcolor{TikTokPink}{\textit{Key Takeaways:}}}}
  \begin{enumerate}[leftmargin=*, label=\arabic*)]
    \item \textbf{Core Concepts:} An overview of the fundamental principles and mechanisms underpinning the method.
    \item \textbf{Foundation and Evidence:} Key principles and empirical evidence, supported by seminal works.
    \item \textbf{Discussion and Insights:} A comprehensive analysis of the method’s core features, advantages, and potential challenges, along with insightful reflections.
  \end{enumerate}
\end{tcolorbox}

\subsubsection{Core Concepts}

Several studies have identified specific \textit{\textbf{Structural Bias}} in Transformer architectures that directly influence the emergence of AS. Two primary sources are causal masking bias and RoPE‑induced bias.

\paragraph{Causal Masking Bias.}
Causal masking forces each token to attend only to previous tokens, creating an inherent advantage for early positions. The first token is visible to all subsequent tokens, while later tokens have progressively fewer opportunities to be attended. This asymmetry systematically biases attention toward the beginning of the sequence, directly inducing AS. Several works have formalized this bias.

\begin{itemize}
    \item \textbf{Position Bias} \cite{wu2025emergence}: Models the causal mask as a graph where early tokens have higher out‑degree, leading to a cumulative attention advantage. Because early tokens receive attention from more queries, the first token inevitably becomes an AS. This structural bias is intrinsic to autoregressive generation.
    
    \item \textbf{Lost in the Middle} \cite{salvatore2025lost}: Observes a U‑shaped position bias (high attention at both ends, low in the middle) and directly attributes the primacy effect to AS. This shows that AS is not an artifact but a key driver of retrieval performance in long‑context tasks.
    
    \item \textbf{A2SF} \cite{jo2024a2sf}: Identifies that causal masking causes early tokens to accumulate artificially high attention scores. Due to causality, the first token’s cumulative score grows much faster than others, systematically overestimating its importance. This directly explains why AS consistently appears at the first token.
\end{itemize}

\paragraph{RoPE-Induced Bias.}
RoPE encodes relative positions by rotating query and key vectors. The resulting attention score depends only on the relative distance between tokens. This relative encoding introduces a structural bias: for certain frequency components, attention decays with distance, concentrating on nearby positions. When this decay is too strong or misaligned with the data, it can create massive activation outliers that distort attention distribution and produce AS. Several works have analyzed this mechanism.

\begin{itemize}
    \item \textbf{What drives attention sinks?} \cite{zhang2026drives}: Shows that RoPE’s one‑dimensional long‑term decay imposes an “image‑alignment bias” on 2D visual tokens linearized into a 1D sequence. This decay forces attention to concentrate on patches that are close in the 1D order but far in the actual 2D image, creating massive activation outliers that produce AS.
    
    \item \textbf{DoPE} \cite{xiong2025dope}: Analyzes RoPE’s frequency spectrum and finds that low‑frequency components lead to low‑rank, over‑aligned attention patterns. The attention matrix becomes nearly rank‑1, with most probability mass concentrated on a single token—the AS. 
    
    \item \textbf{RoPE Weight Angle} \cite{chen2024rotary}: Reveals that the angle between query and key weight vectors determines positional preference. When the weight vectors are non‑orthogonal, the attention logit becomes a function of the relative distance, causing attention to concentrate on specific relative offsets. This can manifest as AS at the first token or other fixed positions.
\end{itemize}

\subsubsection{Foundation and Evidence}

\paragraph{Observational Evidence.}
Several studies have directly observed that structural biases lead to AS.

\begin{itemize}
    \item \textbf{Position Bias} \cite{wu2025emergence}: Using a graph‑theoretic analysis, the authors show that the causal mask inherently biases attention toward early positions. Deep-layer tokens increasingly attend to early tokens, which accumulate richer representations. Figure~\ref{fig:wu_attention_distribution} visualizes this trend across layers.
    
    \item \textbf{Lost in the Middle} \cite{salvatore2025lost}: Training GPT‑2 and Llama models from scratch with controlled long‑term and short‑term memory demands produces a U‑shaped accuracy curve across token positions (see Figure~\ref{fig:salvatore_u_shape}). The primacy effect is directly attributed to the attention sink phenomenon.
    
    \item \textbf{A2SF} \cite{jo2024a2sf}: Due to causality, early tokens accumulate artificially high cumulative attention scores. Figure~\ref{fig:a2sf_accumulation} plots the cumulative score \(S_j^{(t)} = \sum_{s=1}^{t} A_{s,j}\) over generation steps, showing that \(S_1^{(t)}\) grows much faster than others.
    
    \item \textbf{What drives attention sinks?} \cite{zhang2026drives}: RoPE’s one‑dimensional long‑term decay imposes an “image‑alignment bias” on linearized 2D visual tokens. This creates massive activations in fixed hidden dimensions (e.g., 1415, 2533), as visualized in Figure~\ref{fig:zhang_massive_activations}. These massive activations distort attention distribution and produce AS.
    
    \item \textbf{DoPE} \cite{xiong2025dope}: Spectral analysis of RoPE reveals that low‑frequency components lead to low‑rank, over‑aligned attention patterns. The attention matrix becomes nearly rank‑1, with most probability mass concentrated on a single token—the AS (see Figure~\ref{fig:dope_spectrum}).
    
    \item \textbf{RoPE Weight Angle} \cite{chen2024rotary}: The angle between query and key weight vectors determines positional preference. Non‑orthogonal pairs cause attention to concentrate on specific relative offsets, as shown in Figure~\ref{fig:chen_angle_effect}. This can manifest as AS at the first token or other fixed positions.
\end{itemize}

\paragraph{Causal Evidence.}
Direct interventions that modify the structural bias confirm its causal role in AS.

\begin{itemize}
    \item \textbf{What drives attention sinks?} \cite{zhang2026drives}: The paper directly replaces RoPE with Manhattan Causal Attention, which uses 2D Manhattan distance instead of 1D rotary decay. This intervention eliminates the “image‑alignment bias” and, as shown in Figure~\ref{fig:zhang_as_elimination}, completely removes the massive activations and the resulting AS. This provides a clear causal link: RoPE’s one‑dimensional decay structure is a direct cause of AS in vision‑language models.
    
    \item \textbf{A2SF} \cite{jo2024a2sf}: By introducing a forgetting factor \(\gamma\) to reduce the cumulative attention advantage of early tokens, the artificially inflated scores of early tokens are suppressed. As shown in Figure~\ref{fig:a2sf_as_suppression}, this intervention weakens the AS phenomenon, confirming that the cumulative bias introduced by causal masking directly contributes to AS.
\end{itemize}

\subsubsection{Discussion and Insights}
